A Pragmatic Non-Blocking Concurrent Directed Acyclic Graph

In this paper, we have developed two algorithms for maintaining acyclicity in a concurrent directed graph. The first algorithm is based on a wait-free reachability query and the second one is based on partial snapshot-based obstruction-free reachability query. Interestingly, we are able to achieve the acyclic property in the dynamic setting without the need of helping using descriptors by other threads or clean double collect mechanism. We present a proof to show that the graph remains acyclic at all times in the concurrent setting. We also prove that the acyclic graph data-structure operations are linearizable. We implement both the algorithms in C++ and test through a number of micro-benchmarks. Our experimental results show an average of 7x improvement over the sequential and global lock implementation.

==> app-fpsp.tex <==
\section{\FPSP}
\label{sec:app-fpsp}
%\input{code/code6.tex}

==> app-model.tex <==
\section{System Model}
\label{sec:app-model}
An \FAA${(x, a)}$ instruction atomically increments the value at the memory location ${x}$ by the value $a$. Similarly, a \texttt{CAS}${(x, a, a')}$ is an atomic instruction that checks if the current value at a memory location ${x}$ is equivalent to the given value ${a}$, and only if true, changes the value of ${x}$ to the new value ${a'}$ and returns \tru; otherwise the memory location remains unchanged and the instruction returns \fal. Such a system can be perfectly realized by a Non-Uniform Memory Access (NUMA) computer with one or more multi-processor CPUs.

==> figs/bfsExp.tex <==
%\vspace{-0.4cm}
\begin{figure}
\setlength{\belowcaptionskip}{-10pt}
\captionsetup{font=scriptsize}
   % \begin{subfigure}[b]{0.92\textwidth}
    \setlength{\belowcaptionskip}{-7pt}
    \captionsetup{font=scriptsize}
    %\caption{Add 50\% \& Rem 50\%}
        \centering
        \resizebox{\linewidth}{!}{
	\begin{tikzpicture} [scale=0.450]
	\begin{axis}[legend style={at={(1.25,1.0)},anchor=north},
	xlabel=No of threads,
	ylabel=Time in Seconds, ylabel near ticks]
	
	\addplot table [x=Threads, y=$Seq-List$]{results/bfs5050.dat};
		\addlegendentry{$Seq\text{-}list$}
	\addplot table [x=Threads, y=$Coarse-List$]{results/bfs5050.dat};
    	    \addlegendentry{$Coarse\text{-}list$}
	\addplot  table [x=Threads, y=$LF-Hash-DC$]{results/bfs5050.dat};
	 \addlegendentry{$LF\text{-}Hash$}
	\addplot  table [x=Threads, y=$LF-List-DC$]{results/bfs5050.dat};
    \addlegendentry{$LF\text{-}list$}
    	\addplot table [x=Threads,
    %\addplot[blue,sharp plot,update limits=false] 
    y=$LF-BST-DC$]{results/bfs5050.dat};
    \addlegendentry{$LF\text{-}BST$}
    %\addplot[scarletred1,sharp plot,update limits=false] 
    	\addplot  table [x=Threads,
    y=$Ligra$]{results/bfs5050.dat};
    \addlegendentry{$Ligra$}
   % \addplot[red,sharp plot,update limits=false] 	coordinates {(-15,28726) (90,28726)} 	node[above] at (axis cs:2,29856) {base-line};
	\end{axis}
	\end{tikzpicture}
        }
       % \label{fig:cgds-90-10}
   % \end{subfigure}
    %\hspace{-0.6mm}
 % \vspace{-6mm}
%\setlength{\belowcaptionskip}{-15pt}
%\caption{Acyclic Graph Data-Structure.} 
\label{fig:accgds}
\end{figure}  
    
    \ignore{
    \begin{subfigure}[b]{0.32\textwidth}
    \setlength{\belowcaptionskip}{2mm}
    \captionsetup{font=footnotesize, justification=centering}
     \caption{Equal Lookup and Update}%Distribution 50-50\%\caption{CV:15\%, CE:15\%, AddE:25\%, DelE:10\%, AddV:25\% \& DelV:10\%.}
    \centering
    \resizebox{\linewidth}{!}{
	\begin{tikzpicture} [scale=0.230]
	\begin{axis}[
    ybar,
   % ymin=1,
    xmin=1,
    xmax=70,
    enlargelimits=0.1,
   % symbolic x coords={1, 10, 20, 30, 40, 50, 60, 70},
   xticklabels={1, 10, 20, 30, 40, 50, 60, 70},
   xlabel near ticks,
   xtick=data,
    bar width=3.5pt,
    legend style={at={(0.5,121,0.97)},anchor=north},
	xlabel=No of threads,
	ylabel=Throughput ops/sec,
    ylabel near ticks]
	\addplot [butter1, fill=butter1] table [x=Threads, y=$Sequential$]{results/ds5050.dat};
	%	\addlegendentry{$Sequential$}
	\addplot[chameleon1,fill=chameleon1] table [x=Threads, y=$Coarse$]{results/ds5050.dat};
	%	    \addlegendentry{$Coarse$}
	\addplot[plum1,fill=plum1] table [x=Threads, y=$Single-Collect$]{results/ds5050.dat};
	\addplot[chocolate1,fill=chocolate1] table [x=Threads, y=$Double-Collect$]{results/ds5050.dat};
    \addplot[blue,sharp plot,update limits=false] 
	coordinates {(-15,11067) (90,11067)} 
	node[above] at (axis cs:2,12067) {base-line};
	%	    \addlegendentry{$VElock-DIELock\text{-}Free$}
	\end{axis}
	\end{tikzpicture}
        }
        \label{fig:cgds-50-50}
    \end{subfigure}
      %  \setlength{\belowcaptionskip}{-2mm}
%\caption{Acyclic Graph Data-Structure.} 
%\label{fig:accgds1}
%\end{figure*}
%\begin{figure*}[tb]
%\captionsetup{font=footnotesize}
    \begin{subfigure}[b]{0.32\textwidth}
    \captionsetup{font=footnotesize, justification=centering}
    %\setlength{\belowcaptionskip}{-2mm}
   \caption{High Update}% Distribution 10-90\%,\caption{AddE:50\%, DelE: 50\% and rest are 0\%}
        \centering
        \resizebox{\linewidth}{!}{
           \begin{tikzpicture}[scale=0.230]
	%\caption{M1}
	\begin{axis}[
    ybar,
   % ymin=1,
    xmin=1,
    xmax=70,
    enlargelimits=0.1,
   % symbolic x coords={1, 10, 20, 30, 40, 50, 60, 70},
   xticklabels={1, 10, 20, 30, 40, 50, 60, 70},
   xlabel near ticks,
   xtick=data,
    bar width=3.5pt,
    legend style={at={(0.621,0.6597)},anchor=north},
	xlabel=No of threads,
	ylabel=Throughput ops/sec,
    ylabel near ticks]
	\addplot [butter1, fill=butter1] table [x=Threads, y=$Sequential$]{results/ds1090.dat};
	%	\addlegendentry{$Sequential$}
	\addplot[chameleon1,fill=chameleon1] table [x=Threads, y=$Coarse$]{results/ds1090.dat};
		    %\addlegendentry{$Coarse$}
	\addplot[plum1,fill=plum1] table [x=Threads, y=$Single-Collect$]{results/ds1090.dat};
	\addplot[chocolate1,fill=chocolate1] table [x=Threads, y=$Double-Collect$]{results/ds1090.dat};
    \addplot[blue,sharp plot,update limits=false] 
	coordinates {(-15,7777) (90,7777)} 
	node[above] at (axis cs:2,7977) {base-line};
		   % \addlegendentry{$Lock\text{-}Free$}
	\end{axis}
	\end{tikzpicture}
        }
        \label{fig:cgds-10-90}
    \end{subfigure}
}




